Contrastive Learning for Label-Efficient Semantic Segmentation

Collecting labeled data for the task of semantic segmentation is expensive and time-consuming, as it requires dense pixel-level annotations. While recent Convolutional Neural Network (CNN) based semantic segmentation approaches have achieved impressive results by using large amounts of labeled training data, their performance drops significantly as the amount of labeled data decreases. This happens because deep CNNs trained with the de facto cross-entropy loss can easily overfit to small amounts of labeled data. To address this issue, we propose a simple and effective contrastive learning-based training strategy in which we first pretrain the network using a pixel-wise, label-based contrastive loss, and then fine-tune it using the cross-entropy loss. This approach increases intra-class compactness and inter-class separability, thereby resulting in a better pixel classifier. We demonstrate the effectiveness of the proposed training strategy using the Cityscapes and PASCAL VOC 2012 segmentation datasets. Our results show that pretraining with the proposed contrastive loss results in large performance gains (more than 20% absolute improvement in some settings) when the amount of labeled data is limited. In many settings, the proposed contrastive pretraining strategy, which does not use any additional data, is able to match or outperform the widely-used ImageNet pretraining strategy that uses more than a million additional labeled images.

==> approach_old.tex <==
\section{Proposed approach}
Typical semantic segmentation models consist of a CNN feature extractor followed by a pixel-wise softmax classifier.\ In this section, we present the proposed approach for training such models in both fully-supervised and semi-supervised settings.
\begin{figure*}[t]
    \centering
    \includegraphics[trim=20 230 60 20,clip,width=0.7\textwidth]{images/seg_approach.pdf}
    \caption{Proposed training strategy in fully-supervised setting: First, we pretrain the feature extractor using a pixel-wise label-based contrastive loss along with a projection head. Then, we add a softmax classifier on top of the pretrained feature extractor and fine-tune the entire network using pixel-wise cross-entropy loss.}
    \label{fig:approach}
\end{figure*}
\subsection{Fully-supervised setting}
\label{sec:fully-supervised}
In this setting, we have access to only pixel-level labeled images with no additional unlabeled images.\ In this case, we first pretrain the CNN feature extractor from scratch with the pixel-wise label-based contrastive loss~\eqref{eqn:loss} using the labeled images.\ Following~\cite{simclr,simclrv2,supcon} we use a projection head while training with contrastive loss, i.e., the features $f_i$ and $\hat{f}_i$ used in loss~\eqref{eqn:loss} are the outputs of a projection head rather than the original feature extractor (see Fig.~\ref{fig:approach}). After contrastive pretraining, we discard the projection head, add a pixel-wise softmax classifier on top of the feature extractor, and fine-tune the entire network with pixel-wise cross-entropy loss using the same labeled images. 

It is crucial to train the entire network in the fine-tuning stage, as there is no interaction between pixels from different images during contrastive pretraining. While contrastive pretraining encourages pixels within an image to cluster according to their class labels, softmax fine-tuning rearranges these clusters so that they fall on the correct side of the appropriate decision boundary. 

\subsection{Semi-supervised setting}
\label{sec:semi-supervised}
In this setting, we have access to both pixel-level labeled and unlabeled images. In this case, we first train a model with labeled images using the fully-supervised approach presented in Sec.~\ref{sec:fully-supervised}. Then, we generate pseudo labels for the unlabeled images by running the trained model on them and thresholding the output predictions. Specifically, we assign a pixel to a class if that class receives the highest score for that pixel and that score is above a threshold $T$. If the model does not produce a score above $T$ for any of the classes for a pixel, then that pixel is ignored. Once we generate pseudo labels for the unlabeled images, we retrain the model on both labeled and pseudo-labeled images using the fully-supervised approach presented in Sec.~\ref{sec:fully-supervised}.
